Representation Learning in Continuous-Time Dynamic Signed Networks

Signed networks allow us to model conflicting relationships and interactions, such as friend/enemy and support/oppose. These signed interactions happen in real-time. Modeling such dynamics of signed networks is crucial to understanding the evolution of polarization in the network and enabling effective prediction of the signed structure (i.e., link signs and signed weights) in the future. However, existing works have modeled either (static) signed networks or dynamic (unsigned) networks but not dynamic signed networks. Since both sign and dynamics inform the graph structure in different ways, it is non-trivial to model how to combine the two features. In this work, we propose a new Graph Neural Network (GNN)-based approach to model dynamic signed networks, named SEMBA: Signed link's Evolution using Memory modules and Balanced Aggregation. Here, the idea is to incorporate the signs of temporal interactions using separate modules guided by balance theory and to evolve the embeddings from a higher-order neighborhood. Experiments on 4 real-world datasets and 4 different tasks demonstrate that SEMBA consistently and significantly outperforms the baselines by up to $80\%$ on the tasks of predicting signs of future links while matching the state-of-the-art performance on predicting the existence of these links in the future. We find that this improvement is due specifically to the superior performance of SEMBA on the minority negative class.

==> old-experiments.tex <==
\vspace{1mm}
\noindent\textbf{Dynamic Link Sign Prediction}.

Following~\cite{derr2018signed,javari2020rose,LiuZ0ZCL021}, we use the area under the ROC curve (\textbf{ROC-AUC}) as our primary evaluation metric. It measures the probability that the classifier ranks a randomly chosen positive instance higher than a randomly chosen negative instance.
% \ks{fpr description is wrong.}
In addition, we also use False Positive Rate (\textbf{FPR}) to measure the performance on the minority class (i.e., negative edges). It is defined as the ratio of number of negative samples the model classified as positive over the total number of negative samples. This is an important metric when the datasets are skewed towards the positive class, as is the case in Table~\ref{tab:dataset_stats}. One can obtain good overall performance by just predicting all links to be positive but this will lead to an FPR of $1$. 
% In addition, we use the false positive rate (\textbf{FPR}), which considers the accuracy for the minority class (i.e., negative links). It measures the ratio of negative samples that a model classified as positive over all the negative samples, i.e., predicting all links to be positive would thus, make the FPR to be $1$, which is undesirable. 
% Note that this metric is important since the datasets are skewed towards the positive class (see $f_{ub}$ in Table~\ref{tab:dataset_stats}). 
% Predicting all links to be positive would thus, make the FPR to be $1$, which is undesirable. 
% \srijan{FPR is an unusual metric, so need to justify. Say that if all are predicted positive, then FPR will be high and flag it.} 
Thus, a model is deemed effective for dynamic link sign prediction when AUC is high and FPR is low.
% and low FPR indicate that a model is effective for link sign prediction. 

\vspace{1mm}
\noindent\textbf{Dynamic Link Signed Weight Prediction}.
For the regression task, we use the two standard metrics, i.e., root mean squared error (\textbf{RMSE}) and Pearson correlation coefficient (\textbf{PCC}). 
RMSE measures how close the predicted and actual weights are, while PCC quantifies the correlation between predicted and true weights. Thus, low RMSE and high PCC indicate that a model is effective for link signed weight prediction. 
In addition, we use KL-divergence~\cite{kullback1951information} (\textbf{KL-div}) to measure the difference between the predicted and the real weight distribution on the test set. 
The distributions are closer when KL-divergence is low and vice-versa. 

\subsubsection{Implementation Details}
We treat all of the \gnn-based models (i.e., except \rwlstm) as encoder modules that take in a batch of interactions and produce embeddings for all the nodes in an input network. 
Then, we predict the sign/signed-weight of the links by passing these embeddings through a dot-product-based \mlp decoder. This is trained in an end-to-end manner via a BCE (i.e., Equation~\ref{eq:loss_sp}) or RMSE (i.e., Equation~\ref{eq:loss}) loss with the Adam optimizer. 
The predictions are made in a temporal batch, i.e., $t_k = t_j + t_b$, where $t_b$ is fixed to be $1,000$ interactions for the smaller \bitcoinotc and \bitcoinalpha datasets, while it is fixed to be $4,000$ interactions for the larger \epinions and \wikirfa datasets.
% All the models were trained using a BCE or RMSE loss with the Adam optimizer and 
% an adaptive learning rate starting at 0.001 and early stopping with a patience of 5. 
The experiments were conducted on the NVIDIA Tesla K$80$ GPUs with $12$GB memory, and the models were implemented using the PyTorch Geometric framework.\footnote{\url{https://github.com/pyg-team/pytorch_geometric}}  

We carefully tuned the hyperparameters of baselines and \name. Specifically, for hyperparameters of the baselines, we used the best settings found via grid search on the validation set. \name was 
% we set its hyperparameters as follows:
% \yc{Please add important paraemter settings of \name.}\mr{Can you check?}
trained using a BCE or RMSE loss with the Adam optimizer, and an adaptive learning rate starting at $0.001$ and early stopping with a patience of $5$. 
Also, $L1$ regularization was also employed during training, with its parameter $\lambda = 0.0001$ giving the best results. 
% \ks{@Mohit to fix this ->}
We use $512$ as the dimension of node embeddings and use $8$ attention head for the transformer. 
% Lastly, we set the dimensionality of node embeddings, the number of GNN layers, and the number of attention heads are 512, 1, and 8, respectively.
% \yc{Don't we have GNN-related parameters? e.g., \# GNN layers} \mr{Please check}
% For obtaining graph embedding, we used a GNN with one Graph Attention layer (cite TransformerConv paper - Masked Label Prediction: Unified Message Passing Model fr Semi-Supervised Classification) of embedding dimension 512 and 8 attention heads. 
% For more details, refer Appendix \ref{app:}

% \vspace{1mm}
% \noindent\textbf{Parameters}. 


% Model-level parameters can be dumped in the appendix. \ks{Mohit, check}

% \subsection{Evaluation metrics}


% The Receiver Operating Curve (ROC) is a probability curve that plots the change in the model's classification performance as the model's classification threshold changes. The area under the ROC curve is a measure of the model's overall classification ability, indicating its effectiveness in separating the two classes during prediction.


% We also noted in our experiments that several models failed to predict negative links during testing, and so, also report the False Positive Rate (\textbf{FPR}) to evaluate its performance on the minority class of negative links. FPR is the ratio of number of negative samples the model falsely predicts as positive, against the total number of negative samples in the evaluation setup. 

% \res{Mohit Write about these here --
% \begin{itemize}
%     \item ROC-AUC
%     \item FPR
% \end{itemize}
% }

% \subsection{Training and Evaluation Setup}
% For each of these datasets, the model gets to train on the first 70\% of the links (in the sequential order). The next 10\% is used as the validation set for hyperparameter tuning and the final 20\% of the links are used for final testing and reporting the performance. 

% All of the \gnn based models (i.e. except \rwlstm) were treated as encoder modules that take in a batch of interaction (links) and produce embeddings for all the nodes involved. These embeddings are then passed through a dot-product based \mlp decoder that predicts the sign of the link. All the models were trained over Binary cross-entropy loss, through the Adam optimiser with a learning rate of 0.001 and scheduled to decrease if performance on validation set doesn't improve for 10 epochs. 

\begin{table}[tb]
    \centering
    \caption{Comparison of performance on dynamic link sign prediction. Higher AUC and lower FPR is desired. Bold values are the best performing and underlined values are the second best. 
    % \srijan{add up and down arrows next to AUC and FPR, respectively, showing that high AUC and low FPR are better.}\ks{Not fitting well. Common metrics anyway}
    }
    \vspace{-0.2cm}
    \renewcommand{\arraystretch}{1}
    \resizebox{0.49\textwidth}{!} {
    \begin{tabular}{c | c c c c c c c c}
    \toprule
    \textbf{Method} & \multicolumn{2}{c}{\textbf{\btcotc}} & \multicolumn{2}{c}{\textbf{\btcalpha}} & \multicolumn{2}{c}{\textbf{\epinions}} & \multicolumn{2}{c}{\textbf{\wikirfa}} \\
    & AUC & FPR & AUC & FPR & AUC & FPR & AUC & FPR \\
    \midrule
    \gcn & 0.53 & 1.00 & 0.60 & 1.00 & 0.70 & 0.98 & \ul{0.55} & 0.99 \\
    
    \sage & 0.61 & 1.00 & 0.60 & 1.00 & 0.69 & 0.99 & 0.51 & 1.00 \\
    
    \sgcn & \ul{0.63} & \ul{0.76} & 0.61 & \ul{0.73} & 0.68 & 0.98 & 0.49 & 1.00 \\
    
    \rwlstm & 0.57 & 1.00 & 0.39 & 1.00 & 0.50 & 0.91 & 0.49 & 1.00 \\ 
    
    \tgn & 0.60 & 0.84 & \ul{0.62} & 0.91 & \ul{0.71} & \ul{0.63} & \textbf{0.62} & \ul{0.90} \\ \midrule
    
    \textbf{\name} & \textbf{0.64} & \textbf{0.64} & \textbf{0.70} & \textbf{0.65} & \textbf{0.76} & \textbf{0.46} & \textbf{0.62} & \textbf{0.81} \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.2cm}
    \label{tab:signpred}
\end{table}

\subsection{Prediction Performance}\label{sec:performance}
In this section, we evaluate the performance of \name against baselines for the tasks of dynamic link sign prediction (Problem~\ref{prob:signpred}) and dynamic link signed weight prediction (Problem~\ref{prob:signwtpred}). 

\begin{table}[tb]
    \centering
    \caption{Comparison of performance on dynamic link sign weight prediction. Lower RMSE, lower KL divergence, and higher PCC is desired.  Bold values are the best performing and underlined values are the second best. }
    \vspace{-0.2cm}
    \renewcommand{\arraystretch}{1}
    \resizebox{0.45\textwidth}{!} {
    \begin{tabular}{c | c c c @{\hskip 2mm} c c c}
    \toprule
    \textbf{Method} & \multicolumn{3}{c}{\textbf{\btcotc}} & \multicolumn{3}{c}{\textbf{\btcalpha}} \\
    & RMSE & PCC & KL div & RMSE & PCC & KL div \\
    \midrule
    \gcn & 9.73 & 0.11 & 24.79 & 9.42 & -0.01 & 10.15 \\
    
    \sage & 11.50 & 0.05 & 25.45 & 9.45 & 0.01 & 24.24 \\
    
    \sgcn & 9.71 & 0.07 & 24.34 & 11.62 & 0.02 & 24.52 \\
    
    \rwlstm & \ul{5.85} & 0.08 & \ul{11.49} & 6.17 & \ul{0.10} & 12.17 \\ 
    
    \tgn & 
    \textbf{3.56} & \textbf{0.13} & \textbf{4.67} & 
    \ul{3.71} & 
    -0.01 & 
    \ul{4.77} \\ \midrule
    
    \textbf{\name} & \textbf{3.56} &
    \ul{0.12} & 
    \textbf{4.67} &
    \textbf{3.35} & \textbf{0.22} &
    \textbf{1.45} \\
    
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.2cm}
    \label{tab:weightpred}
\end{table}

\subsubsection{Dynamic Link Sign Prediction}
Table~\ref{tab:signpred} illustrates the results on dynamic link sign prediction. The values in bold face and underlined indicate the best and $2$nd best performing methods in each column, respectively. We can make multiple observations based on these results.
% We summarize the results shown in Table~\ref{tab:signpred} as follows.
% As noted above, this task is inherently hard to solve, because of a combination of factors like a majority of nodes being unseen during training, staleness of the embeddings produced and extreme imbalance in sign distribution. 

First, \name significantly outperforms or matches the performance of the baselines in all cases.
Specifically, on \epinions dataset, \name yields up to $6.57$\% higher AUC and $26.98$\% lower FPR than the strongest baseline \tgn.
The results indicate that modeling balance and network evolution together is effective in accurately predicting signs of future links.
Second, among the baselines, we see that for the smaller \btcotc and \btcalpha datasets, the baseline for signed networks (i.e., \sgcn) came closest to our model while for larger \wikirfa and \epinions datasets, the baseline for dynamic networks (i.e., \tgn) beats \sgcn. 
For large dynamic networks, we attribute the superiority of \tgn to its modeling of the temporal order (C1) between the links in addition to avoiding the staleness (C2) problem in these large but sparse networks. 
% its handling the temporal 
% information 
% in addition to the sign information, 
% thereby avoiding the staleness problem. 

% Lastly, we examine the results on FPR in detail. 
Furthermore, we see that the difference in performance with respect to FPR between \name and baselines is quite drastic, especially in more imbalanced datasets such as \btcotc, \btcalpha, and \epinions (see Table \ref{tab:dataset_stats}). 
\name obtains a reduction in FPR of at least $0.09$ and up to $0.17$ from the baselines. 
The unsigned baselines (i.e., \gcn and \sage) are found to give a high FPR of $\sim 1$ across datasets, indicating that they fail to learn the sign structure of the links and only predict the majority positive sign for all links. 
\sgcn obtains good performance on the small datasets (\btcotc and \btcalpha) becoming the second best approach but fails to model the sign structure in larger datasets. This can be attributed to the fact that \sgcn does not handle the temporal order (C1) and staleness (C2) of embeddings that becomes important on larger and sparser datasets such as \epinions and \wikirfa. In other words, modeling temporal order becomes important to predict signs of future links when the links are sparse in a dataset. 
This is evident by the superior performance of \tgn in these larger datasets. On the other hand, \tgn fails to accurately predict negative links on the smaller datasets where it gets beaten by \sgcn. This shows that balance theory is important to represent links for sign prediction tasks when the network is smaller (but denser). Finally, \name outperforms these baselines in all the cases indicating that jointly modeling time and balance theory consistently gives significant improvement in performance. 

% \yc{The descriptions below are unclear, and are written in terms we haven't mentioned before. The experiment section should be a part that demonstrates the claims made in the previous sections, not a new claim.}\ks{What is the new claim ? We are explaining the performance in FPR. Remove the scarcity comment if that's better.}
% \yc{It would be better if we can directly use C1, C2, and C3 mentioned in Section 1. Further, we need to write the limitations of baselines more clearly; please check the comments below.}
% In fact, one can observe that all models tend to predict positive links leading to a high false positive rate. 
% In many applications such as predicting conflicts and distrust relations, it could be very crucial to accurately predict the negative links, despite their low number. 
% There is scarcity of negative links in all datasets, which is exacerbated in the dynamic setting since one is provided with only the historical structure to make future prediction.\yc{TGN doesn't only use the historical structure.}
% In the dynamic setting, this problems becomes even harder as we see from the low FPR of most static models since the history might not include many negative interactions to learn enough. 
% Explicitly exploiting connectivity biases like balance theory in modeling history allows us to learn in a more data-efficient manner as is evident from the superior performance of \name.\yc{SGCN explicit exploits connectivity biases like balance theory.}

% \yc{Another discussion point -- reviewers may wonder why FPRs of SGCN and RW-LSTM are significantly high, even though they consider the link signs.
% In this regard, we can claim that these results indicate their poor inductive capability; Table 6 can support such a claim.}
% However, these explicit biases could also lead to incorrect generalization as we see from the lower performance on \wikirfa. This can be explained by noting that \wikirfa has comparatively a much higher fraction of unbalanced triangles than the other datasets, which could explain the comparatively higher FPR. 
% This is expected, since these models are expressively designed keeping in mind the whole graph structure. \tgn shows slightly better performance, but our model largely outperforms all the baselines on the Negative links. 

% Balance theory explicitly uses the immediate inter-community substructure, and so our model performs the best on negative link prediction on the more balanced and polarised datasets like the Bitcoin datasets, but has a lot of room for improvement in relatively unbalanced and unpolarised \wikirfa dataset. 

\begin{comment}

\begin{table*}[h]
    \centering
    \caption{ROC-AUC scores for link sign prediction}
    \begin{tabular}{l c @{\hskip 2mm} c @{\hskip 2mm} c @{\hskip 2mm} c}
    \toprule
    \textbf{Method} & \textbf{\btcotc} & \textbf{\btcalpha} & \textbf{\epinions} & \textbf{\wikirfa} \\
    \midrule
    \gcn & 0.5317 & 0.6041 & 0.5505 & 0.5545 \\
    
    \sage & 0.6142 & 0.6045 & 0.5844 & 0.5144 \\
    
    \sgcn & 0.6283 & 0.6074 & 0.5745 & 0.4964 \\
    
    \rwlstm & 0.5693 & 0.3877 & 0.5004 & 0.4995 \\ 
    
    \tgn & 0.6045 & 0.6245 & 0.7542 & 0.6160 \\
    
    \textbf{\name} & \textbf{0.6436} & \textbf{0.7045} & \textbf{0.7574} & \textbf{0.6171} \\
    
    \bottomrule
    \end{tabular}
    \label{tab:roc_auc_scores}
\end{table*}



\begin{table*}[h]
    \centering
    \caption{FPR for link sign prediction}
    \begin{tabular}{l c @{\hskip 2mm} c @{\hskip 2mm} c @{\hskip 2mm} c}
    \toprule
    \textbf{Method} & \textbf{\btcotc} & \textbf{\btcalpha} & \textbf{\epinions} & \textbf{\wikirfa} \\
    \midrule
    \gcn & 1.0000 & 1.0000 & 1.0000 & 0.9982 \\
    
    \sage & 1.0000 & 1.0000 & 0.9924 & 1.0000 \\
    
    \sgcn & 0.7642 & 0.7255 & 0.9884 & 1.0000 \\
    
    \rwlstm & 1.0000 & 1.0000 & 1.0000 & 1.0000  \\ 
    
    \tgn & 0.8374 & 0.9138 & 0.7904 & 0.9040 \\
    
    \textbf{\name} & \textbf{0.6428} & \textbf{0.4465} & \textbf{0.4635} & \textbf{0.8090} \\
    
    \bottomrule
    \end{tabular}
    \label{tab:fpr_scores}
\end{table*}


Table \ref{tab:roc_auc_scores} shows the results of link sign prediction with respect to the ROC-AUC score. Our method matches or outperforms all the baselines on all the datasets we experimented on. It is also interesting to note that for the smaller Bitcoin graphs, the signed baseline (\sgcn) came closest to our model. However, for larger graphs, the dynamic graph method \tgn beats the signed baselines, signalling that for large dynamic graphs, effectively handling the temporal information in addition to sign information is crucial, to avoid the staleness problem. 

Table \ref{tab:fpr_scores} compares the performance of all the models with respect to their False Positive Rate (FPR). This is especially important because high scores on metrics like F1 score or Accuracy can hide the inability of the model to effectively predict the negative links. Signed graphs are an highly imbalanced, and in most applications it is important to get the predictions on the negative links right. In the dynamic setting, when the models see only a small batch of interactions at a time, all the signed models struggle to predict any negative link at all. This is expected, since these models are expressively designed keeping in mind the whole graph structure. \tgn shows slightly better performance, but our model largely outperforms all the baselines on the Negative links. 

Balance theory explicitly uses the immediate inter-community substructure, and so our model performs the best on negative link prediction on the more balanced and polarised datasets like the Bitcoin datasets, but has a lot of room for improvement in relatively unbalanced and unpolarised \wikirfa dataset. 

\end{comment}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/weight_dist.png}
    \caption{Distribution of \name's predicted link signed weights (rounded to the nearest integer) and the true link signed weights on the test set.}
    % \yc{If we run out of space, we can show the results of Bitcoin-Alpha only.}}
    \label{fig:weight_dist}
\end{figure}

\subsubsection{Dynamic Link Signed Weight Prediction}
Table~\ref{tab:weightpred} illustrates the results on dynamic link signed weight prediction. Note that only \bitcoinotc and \bitcoinalpha datasets have link weights.   
We summarize the results shown in Table~\ref{tab:weightpred} as follows.

First, \name outperforms all the baselines in both datasets. 
The results indicate that our design choices contribute to accurately predict not only the sign but also the signed weight of the link.
Second, we see that the dynamic-graph models (\tgn, \rwlstm, \name) completely outperform all the static graph models (\gcn, \sage, \sgcn) in this task. 
This shows that effectively handling temporal information (by overcoming challenges C1 and C2) in a signed dynamic graph is crucial to learn the signed weight distribution on future links. 
% This is consistent with the results shown in Table~\ref{tab:signpred}.
% Therefore, one notes that effectively handling temporal information in a signed dynamic graph is crucial to do sign inference on future links. 
% Furthermore, Table \ref{tab:weightpred} also shows the KL divergence between the distribution of link weight predicted by the model and the true link weights for the \btcalpha test set. 
Low RMSE and KL-divergence shows that \name's predicted link weight distribution is able to best predict the true link weight distribution. This indicates that modeling balance theory by overcoming the challenge C1 allows us to further improve the performance on this task. 
% This is given by our model having the smallest KL divergence between the predicted and true link signed weight distributions. 
% Furthermore, we investigate the KL-div results of \name using Figure~\ref{fig:weight_dist}.
% Next, we compare the distribution of the predicted signed weights with the actual distribution. The distribution predicted by \name gives the lowest KL-divergenece among all the methods. 
We further visualize the distributions of the predicted signed weights and those of the actual signed weights in Figure \ref{fig:weight_dist}.
% by plotting a histogram for \name's prediction against true weights. 
We note that the predicted distribution closely matches the true distribution by being centered around $1$ and gradually decreasing on both sides. However, one can note that the predicted weights fail to predict higher magnitude weights. 
In particular, the model is not able to predict the spike at the negative end of the spectrum, i.e., the high number of links with weight as $-10$ in the real distribution. Since we minimize the RMSE loss during training, the model learns a smooth curve around the center of the distribution, ignoring the outliers at the ends. 
% \yc{I still think that we should discuss the expected reasons for this phenomenon. It is not a small amount to refer to as outliers.}
% The actual distribution of the weights is highly skewed, with a majority of edge weights being positive. Most of the edge are distributed between $[-3, 3]$, with decreasing number of links as the edge weight increases. This shows that people don't express mutual trust/distrust sentiments with a strong effect. Figure \ref{fig:weight_dist} shows that \name's distribution of predicted link weights closely matches the distribution of true link weights, being centered around $1$ and gradually decreasing on both sides. However, one can note that the predicted weights fail to predict higher magnitude weights. In particular, the model is not able to predict the anomalous spike at the negative end of the spectrum, i.e., the high number of links with weight as $-10$ in the real distribution. 
% predict a lot of the higher weights \mr{Any justification? Maybe that the sudden spike in weights -10 and 10 means they are mostly an anomaly and hard for the model to digest?}. 
% One also notes a considerable spike at the tail ends of both positive and negative weights, which correspond to 

% The results for the two problems shows that our dynamic link sign prediction setup (a classification task), with minimal modifications could be adapted for auxiliary tasks like dynamic link signed weight prediction (a regression task). This indicates that the model can function as a general purpose encoder for dynamic signed graph and their associated tasks.









\subsection{Inductive Capability}\label{sec:inductive}
\label{sec:inductive}
% \srijan{move this and associated tables before runtime.}
We note that our problems have the inductive nature since the timeline of the datasets spans several years, with several new users added to the network over the course of these years. 
In particular, Table~\ref{tab:new_nodes} shows the fraction of new nodes in the validation and test sets, which indicates the inherent inductive nature of dynamic prediction in these tasks. 
% which indicates that the validation and test sets  demonstrated in Table~\ref{tab:new_nodes}.
% As mentioned in Section~\ref{sec:intro}, therefore, \name should be able to generalize new nodes and links effectively.
% As shown in Table \ref{tab:new_nodes}, the problem of dynamic link sign prediction is inherently tricky to solve. 
Roughly half of the nodes in the validation setup are unseen during training and over two-thirds of the nodes in testing set are unseen during training. 
% This could be because the timeline of these graph datasets span several years, with several new users added to the network over the course of these years. 
This necessitates the model to be very effective against the cold start problem. 
\yc{Can we briefly introduce how to generate the embeddings of unseen nodes, which is pointed out by WSDM's reviewer?}

\begin{table}[t]
    \centering
    \caption{Fraction of new nodes in the validation and test sets}
    \vspace{-0.2cm}
    \renewcommand{\arraystretch}{1}
    \resizebox{0.45\textwidth}{!} {
    \begin{tabular}{c | c c c c}
    \toprule
    \textbf{Split} & \textbf{\btcotc} & \textbf{\btcalpha} & \textbf{\epinions} & \textbf{\wikirfa} \\
    \midrule
    Val & 0.51 & 0.52 & 0.60 & 0.57 \\
    Test & 0.65 & 0.62 & 0.73 & 0.76 \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.2cm}
    \label{tab:new_nodes}
\end{table}


Table~\ref{tab:inductive} shows the inductive capability of \name, which indicates its performance on sign prediction when the link to be predicted has zero or one or both nodes unseen during the training (denoted by Zero/One/Two unseen in the table respectively). % nodes (i.e., zero/one/two unseen). 
We note that \name performs well in all the cases, even when both end-nodes are unseen during training. %(i.e., two unseen). 
The results thus show that \name effectively addresses the cold-start problem. 
\name owes this inductive capability to its memory update and embedding generator modules that update the representations of new nodes during test phase to encode past interactions and handle staleness respectively. 
% This helps tackle the cold start problem. 
% \yc{I think the descriptions below should be addressed in the proposed method section, not here.}\ks{Removed.}
% During inference, if new nodes occur, \name is able to gather the requisite information from its associated graph structure using balance theory and generate embeddings that can effectively do link sign prediction. 
% As time progresses, the new node participates in new events, which, in turn, updates its memory and embeddings. 
% Furthermore, any interaction in the k-hop neighborhood updates the node embeddings as well.
% This allows \name to effectively utilise the graph structure and interaction history to make informed predictions involving new nodes. 

\begin{table}[t]
    \centering
    \caption{Performance of \name on dynamic link sign prediction task across test sets in which the links have zero, one, and two new nodes.}
    \vspace{-0.2cm}
    \renewcommand{\arraystretch}{1}
    \resizebox{0.49\textwidth}{!} {
    \begin{tabular}{l | c c c c c c c c}
    \toprule
     & \multicolumn{2}{c}{\textbf{\btcotc}} & \multicolumn{2}{c}{\textbf{\btcalpha}} & \multicolumn{2}{c}{\textbf{\epinions}} & \multicolumn{2}{c}{\textbf{\wikirfa}} \\
     & AUC & FPR & AUC & FPR & AUC & FPR & AUC & FPR \\
    \midrule
    Zero unseen &  0.66 & 0.54 & 0.73 & 0.51 & 0.80 & 0.35 & 0.66 & 0.76\\    
    
    One unseen & 0.64 & 0.64 & 0.73 & 0.60 & 0.78 & 0.48 & 0.61 & 0.75 \\
    
    Two unseen & 0.62 & 0.80 & 0.69 & 0.79 & 0.61 & 0.64 & 0.62 & 0.98 \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.2cm}
    \label{tab:inductive}
\end{table}

\subsection{Scalability Analysis}\label{sec:scalability}
\label{sec:runtime}
To test the scalability of \name, we examine the change of the inference time with increase in the size of the dataset. In particular, we note the average prediction time in different datasets (\btcalpha: $10$e4, \wikirfa: $10$e5, \epinions: $10$e6 edges). Figure~\ref{fig:scaling} shows that \sgcn scales at a much higher slope than the other methods, while \name scales at a similar rate with \tgn and other static \gnns.
The results show that \name has a linear scalability with the increasing number of edges in the dataset, which is at par with more efficient unsigned GNN baselines. 
% Furthermore, considering the significant improvement of \name in accuracy over all baselines (see Tables~\ref{tab:signpred} and~\ref{tab:weightpred}), this relatively-slow inference time is still worthwhile.
% \yc{We need to explain more about how we conducted this experiment. Did we randomly sample links from Epinions?}
% \ks{check, we can also remove this section. Does not add much.}
% \yc{If this section is removed, reviewers may point out that the number of experiments is too small.}
% are plotted against the ROC-AUC score of the models, thus showing the trade-off between speed and performance. 
% From Figure~\ref{fig:scaling}, we see that \sgcn scales at a much higher slope than the other methods, while \name scales at a similar rate with \tgn and other static \gnns.
% The results show that \name has a linear scalability with the increasing number of links.
% Furthermore, considering the significant improvement of \name in accuracy over all baselines (see Tables~\ref{tab:signpred} and~\ref{tab:weightpred}), this relatively-slow inference time is still worthwhile.

% On the other hand, \name is only $\sim$ 20 $\mu s$ slower than the second-best performing baseline \tgn in terms of prediction accuracy.


% and gives around $0.2$ increase in the performance. 
% that at the slight cost of slower performance, \name has much better predictive performance.  

% Figure \ref{fig:scaling} shows how inference time per link scales with the size of the dataset graph, in terms of the number of links. All models scale linearly with the dataset size. \sgcn scales at a much higher slope than the other methods. \name scales at a similar rate with \tgn and other static \gnns. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/runtime.png}
%     \caption{Time taken per link for link sign prediction on the \epinions graph test set.}
%     % \srijan{font size still needs to be increased.}\mr{Done}}
%     \label{fig:runtime}
% \end{figure}





% \subsection{Link Signed Weight Distribution}
% \label{sec:weight_dist}

% Figure \ref{fig:weight_dist} shows the distribution of \name's predicted link signed weights (rounded off to the nearest integer) and true link signed weights for the \btcotc and \btcalpha test set. Although the link weights range from -10 to +10, the distribution is highly skewed towards smaller positive and negative values, except for a noticeably large number of links having -10 weights which our model fails to capture. 

==> sec-background.tex <==
\section{Background}



\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/balance.png}
    \caption{Background: Formation of balanced and unbalanced triad as dictated by balance theory}
    \label{fig:balance}
\end{figure}

\subsection{Structural Balance}
Structural balance theory \cite{cartwright1956structural} generalizes Heider's balance theory of attitude change \cite{heider2013psychology} to apply it in any graph-structured data. Many interpersonal relationships and online interactions can be modeled using structural balance \cite{leskovec2010predicting,leskovec2010signed}. This theory asserts that signed links are formed in order to create certain higher-order combinations, called \textit{balanced} states. A triad formed by the nodes $u, v, w$ is balanced if the product of the signs of the edges is positive, i.e. either all edges are positive or exactly two of them are negative. In other words, it asserts four rules: (1) a friend of a friend is a friend, (2) an enemy of a friend is an enemy, (3) enemy of an enemy is a friend, and (4) enemy of a friend is an enemy. The four possible triads are visualised in Figure \ref{fig:balance}. 
% \srijan{Add a visual showing balanced vs unbalanced triads.}\ks{Updated.}


% \srijan{the following reads like related work. Here, you should talk about things that you are using. Other concepts can be moved to the related work.}\ks{Can't do much. We don't have related work and the following paragraph is important.} \srijan{if you are not directly using this, move this to related work section. or remove. }\ks{I think we do use a dynamic tendency towards balanced structures so this should be good.}
Balance theory has also been extended to dynamic structures where links evolve over time. 
% \srijan{I misclaimed in introduction that this has not been done. Pls fix it.}\ks{Couldn't find where. "not clear how" is okay}
A movement toward completion of balanced triads is desired as new positive or negative links become established and the links may be deleted to adjust for balance when unbalanced triads are formed \cite{abell1968structural}. Models have been proposed where new links are added based on random selection of nodes followed by deletions to adjust for balanced structures \cite{abell2009structural}. These simulations provide initial results to model dynamics of signed social networks. 

% \srijan{This is not relevant here. This section is background work. Move elsewhere.} In this work, we present a data-driven approach to represent temporally-evolving signed links by exploiting balance theory to aggregate information from the temporal neighbors. 

% In particular, we use a relaxed form of structural balance where we distinguish between information coming from balanced and unbalanced paths \cite{derr2018signed}. \srijan{you can give more details about this paper and how it works/aggregates. Don't use equations, but textual.}


% Balance theory was proposed as a theory to explain attitude change in psychology \cite{}. It asserts that a balance must exist in interpersonal relationships. 

\subsection{Temporal Graph Networks}
% \srijan{this paragraph is perfect -- it is concise, speaks only about the model that is relevant, and explains it clearly.}
Learning on temporally-evolving graphs require one to effectively encode both graph structure and graph dynamics. Continuous-time dynamic graph models encode time-stamped events such as edge addition/deletion, to update node embeddings over time. Temporal Graph Network (\tgn) \cite{rossi2020temporal} is the state-of-the-art model to learn representations of dynamic graphs. \tgn proposes a general-purpose temporal graph encoder to update embeddings based on a batch of temporal interactions. This model consists of three core modules ---
\begin{enumerate}[leftmargin=*]
    \item \textbf{Message generation:} Interactions/events are encoded using a Multi-Layer Perceptron on the interaction nodes, 
    \item \textbf{Memory:} Each node maintains a memory of events that is updated, using a LSTM or a GRU, upon the occurrence of a new event involving that node, and
    \item \textbf{Embedding:} Temporal emebddings of each node are updated by using temporal graph attention to update information from $k$-hop neighborhood, which allows to avoid memory staleness problem. 
\end{enumerate}
